Code Perfumes: Reporting Good Code to Encourage Learners

Block-based programming languages like Scratch enable children to be creative while learning to program. Even though the block-based approach simplifies the creation of programs, learning to program can nevertheless be challenging. Automated tools such as linters therefore support learners by providing feedback about potential bugs or code smells in their programs. Even when this feedback is elaborate and constructive, it still represents purely negative criticism and by construction ignores what learners have done correctly in their programs. In this paper we introduce an orthogonal approach to linting: We complement the criticism produced by a linter with positive feedback. We introduce the concept of code perfumes as the counterpart to code smells, indicating the correct application of programming practices considered to be good. By analysing not only what learners did wrong but also what they did right we hope to encourage learners, to provide teachers and students a better understanding of learners' progress, and to support the adoption of automated feedback tools. Using a catalogue of 25 code perfumes for Scratch, we empirically demonstrate that these represent frequent practices in Scratch, and we find that better programs indeed contain more code perfumes.

==> tables/Bugpattern_table.tex <==
\begin{table}
\centering
\caption{Number of bugpattern instances found in total and number of projects containing the bugpattern.}
\label{tab:bugpattern_table}
\begin{tabular}{lrrr}
\toprule
                            Bugpattern & \# Patterns & \# Projects &  AVG WMC \\
\midrule
      Ambiguous Custom Block Signature &        326 &         98 &   253.24 \\
         Ambiguous Parameter Name Used &         10 &          8 &    32.62 \\
                      Blocking If Else &        236 &        121 &   429.58 \\
               Call Without Definition &        483 &        142 &   263.31 \\
                    Comparing Literals &      4,774 &      1,843 &   238.93 \\
             Custom Block With Forever &        560 &        170 &   385.55 \\
         Custom Block With Termination &        412 &        108 &   264.75 \\
                     Endless Recursion &        827 &        441 &   124.85 \\
       Expression As Touching Or Color &      1,718 &        384 &   248.54 \\
                   Forever Inside Loop &      5,150 &      1,605 &   202.11 \\
            Illegal Parameter Refactor &          1 &          1 &    17.00 \\
Immediate Delete Clone After Broadcast &      1,899 &        879 &   262.00 \\
        Immediate Stop After Say Think &        220 &        154 &    77.42 \\
    Inappropriate Handler Delete Clone &        907 &        534 &   178.39 \\
              Interrupted Loop Sensing &     61,528 &      9,437 &   142.23 \\
                Message Never Received &     14,836 &      5,575 &   153.24 \\
                    Message Never Sent &     23,298 &      4,291 &   194.42 \\
                           Missing Ask &         88 &         42 &    56.38 \\
               Missing Backdrop Switch &      3,378 &        761 &   111.55 \\
                    Missing Clone Call &      1,050 &        466 &   315.77 \\
          Missing Clone Initialization &      5,470 &      1,587 &   170.46 \\
                     Missing Erase All &        243 &         86 &    62.30 \\
                Missing Initialization &    267,638 &     38,368 &    62.41 \\
                  Missing Loop Sensing &     36,583 &      6,613 &   148.95 \\
                      Missing Pen Down &        229 &        150 &   214.85 \\
                        Missing Pen Up &      2,722 &        972 &    42.68 \\
                      Missing Resource &     20,236 &      6,090 &   161.16 \\
                   Missing Termination &      1,477 &        642 &   216.02 \\
                Missing Wait Condition &        542 &        299 &   361.12 \\
                    No Working Scripts &        682 &        530 &    72.64 \\
                    Orphaned Parameter &        241 &        119 &   361.79 \\
                Parameter Out Of Scope &      2,706 &        719 &   328.30 \\
                 Position Equals Check &     12,439 &      2,435 &   207.00 \\
                     Recursive Cloning &      1,725 &        388 &   251.07 \\
                   Stuttering Movement &     34,804 &      9,934 &    34.11 \\
                       Terminated Loop &      1,548 &        679 &   156.05 \\
                            Type Error &        222 &        137 &   231.14 \\
                   Variable As Literal &     65,998 &      2,814 &   258.24 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/Bugpattern_without_loose_table.tex <==
\begin{table}
\centering
\caption{Number of bugpattern instances found in total and number of projects containing the bugpattern disregarding loose blocks.}
\label{tab:bugpattern_without_loose_table}
\begin{tabular}{lllr}
\toprule
                            Bugpattern & \# Patterns & \# Projects &  AVG WMC \\
\midrule
      Ambiguous Custom Block Signature &        326 &         98 &   253.24 \\
         Ambiguous Parameter Name Used &         10 &          8 &    32.62 \\
                      Blocking If Else &        232 &        119 &   432.08 \\
               Call Without Definition &        253 &        112 &   301.40 \\
                    Comparing Literals &      1,858 &        548 &   242.79 \\
             Custom Block With Forever &        547 &        167 &   389.06 \\
         Custom Block With Termination &        411 &        107 &   261.59 \\
                     Endless Recursion &        827 &        441 &   124.85 \\
       Expression As Touching Or Color &      1,609 &        348 &   264.17 \\
                   Forever Inside Loop &      4,703 &      1,564 &   202.73 \\
            Illegal Parameter Refactor &          1 &          1 &    17.00 \\
Immediate Delete Clone After Broadcast &      1,866 &        872 &   263.50 \\
        Immediate Stop After Say Think &        213 &        149 &    78.70 \\
    Inappropriate Handler Delete Clone &        904 &        532 &   179.06 \\
              Interrupted Loop Sensing &     60,861 &      9,388 &   142.25 \\
                Message Never Received &     12,974 &      5,214 &   151.74 \\
                    Message Never Sent &     26,949 &      4,768 &   188.62 \\
                           Missing Ask &         55 &         18 &   188.33 \\
               Missing Backdrop Switch &      3,675 &        804 &   116.96 \\
                    Missing Clone Call &      1,545 &        642 &   291.52 \\
          Missing Clone Initialization &      4,687 &      1,452 &   166.57 \\
                     Missing Erase All &        428 &        122 &    45.20 \\
                Missing Initialization &    238,976 &     34,762 &    64.13 \\
                  Missing Loop Sensing &     36,384 &      6,588 &   148.88 \\
                      Missing Pen Down &        247 &        157 &   204.87 \\
                        Missing Pen Up &      2,595 &        956 &    41.67 \\
                      Missing Resource &     17,333 &      5,585 &   163.05 \\
                   Missing Termination &      1,017 &        347 &   187.26 \\
                Missing Wait Condition &        230 &         91 &   376.30 \\
                    No Working Scripts &        682 &        530 &    72.64 \\
                    Orphaned Parameter &        241 &        119 &   361.79 \\
                Parameter Out Of Scope &        280 &        108 &   183.01 \\
                 Position Equals Check &     12,032 &      2,384 &   208.11 \\
                     Recursive Cloning &      1,723 &        386 &   252.37 \\
                   Stuttering Movement &     34,817 &      9,945 &    35.25 \\
                       Terminated Loop &      1,512 &        659 &   150.08 \\
                            Type Error &        156 &         87 &   250.77 \\
                   Variable As Literal &     62,261 &      2,751 &   261.92 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/Perfume_without_loose_table.tex <==
\begin{table}
\centering
\caption{Number of perfume instances found in total and number of projects containing the perfume disregarding loose blocks.}
\label{tab:perfume_without_loose_table}
\begin{tabular}{lllr}
\toprule
                    Perfume & \# Patterns & \# Projects &  AVG WMC \\
\midrule
            Backdrop Switch &    140,220 &      8,612 &    73.45 \\
         Boolean Expression &  1,003,173 &     34,845 &    77.48 \\
                  Collision &     59,013 &     14,418 &    72.23 \\
               Coordination &     64,613 &     10,017 &   132.35 \\
          Correct Broadcast &    285,781 &     37,158 &    70.92 \\
         Custom Block Usage &    164,445 &      9,634 &   116.07 \\
            Directed Motion &      8,039 &      2,116 &    30.01 \\
             Gliding Motion &      7,294 &      1,810 &    43.44 \\
    Initialisation of Looks &    473,486 &     54,055 &    57.67 \\
Initialisation of Positions &    132,149 &     39,055 &    62.74 \\
                 List Usage &    122,336 &      4,000 &   172.17 \\
        Matching Parameters &     50,573 &      4,668 &   152.59 \\
             Mouse Follower &      5,412 &      4,009 &    73.61 \\
           Movement In Loop &     14,800 &      8,440 &    76.19 \\
       Nested Loops Perfume &     29,832 &     11,247 &   116.92 \\
            Object Follower &      9,671 &      3,948 &   146.80 \\
            Parallelization &  1,141,278 &     70,509 &    49.74 \\
  Say Sound Synchronization &        154 &         40 &    85.80 \\
                      Timer &     20,510 &     12,949 &   103.78 \\
      Useful Position Check &     27,831 &      7,378 &   125.50 \\
          Valid Termination &     77,278 &     16,298 &   105.34 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/Smell_table.tex <==
\begin{table}
\centering
\caption{Number of smell instances found in total and number of projects containing the smell.}
\label{tab:smell_table}
\begin{tabular}{lrrr}
\toprule
                           Smell & \# Patterns & \# Projects &  AVG WMC \\
\midrule
 Ambiguous Parameter Name Unused &         50 &         41 &    98.76 \\
                    Busy Waiting &     19,373 &      7,202 &   117.62 \\
                    Clone Type 1 &    194,445 &      7,118 &   181.23 \\
                    Clone Type 2 &    324,476 &     12,052 &   140.72 \\
                    Clone Type 3 &  1,049,424 &     11,197 &   142.07 \\
                       Dead Code &    155,130 &     23,294 &    87.13 \\
                       Double If &      5,106 &      1,381 &   306.32 \\
                Duplicate Sprite &    719,411 &     12,365 &    73.88 \\
               Duplicated Script &     23,130 &      8,820 &   142.15 \\
              Empty Control Body &     35,254 &      8,723 &   145.17 \\
              Empty Custom Block &      2,003 &      1,075 &   203.20 \\
                   Empty Project &         27 &         27 &     0.00 \\
                    Empty Script &     24,075 &      9,979 &   115.96 \\
                    Empty Sprite &     25,858 &     11,341 &    53.58 \\
                     Long Script &    139,536 &     34,086 &    75.64 \\
                  Message Naming &    198,420 &     15,852 &    81.23 \\
                      Middle Man &      1,578 &        905 &   342.08 \\
Multiple Attribute Modifications &     13,243 &      4,305 &   172.40 \\
                    Nested Loops &      7,037 &      1,813 &   164.43 \\
  Same Variable Different Sprite &     67,485 &      3,633 &   239.78 \\
              Sequential Actions &      9,848 &      3,235 &   151.46 \\
                   Sprite Naming &    222,684 &     47,715 &    58.14 \\
      Unnecessary If After Until &        985 &        452 &   151.61 \\
                Unnecessary Loop &      4,603 &      1,703 &   176.24 \\
                Unnecessary Time &     27,295 &      3,841 &   169.89 \\
             Unused Custom Block &      6,214 &      2,139 &   196.66 \\
                Unused Parameter &      3,361 &      1,363 &   212.90 \\
                Unused Variables &     67,398 &     11,577 &   122.65 \\
    Variable Initialization Race &      9,673 &      5,583 &   183.42 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/Smell_without_loose_table.tex <==
\begin{table}
\centering
\caption{Number of smell instances found in total and number of projects containing the smell disregarding loose blocks.}
\label{tab:smell_without_loose_table}
\begin{tabular}{lllr}
\toprule
                           Smell & \# Patterns & \# Projects &  AVG WMC \\
\midrule
 Ambiguous Parameter Name Unused &         50 &         41 &    98.76 \\
                    Busy Waiting &     19,089 &      7,133 &   115.91 \\
                    Clone Type 1 &    163,076 &      6,675 &   184.28 \\
                    Clone Type 2 &    302,425 &     11,832 &   142.16 \\
                    Clone Type 3 &    981,920 &     10,985 &   142.82 \\
                       Dead Code &    154,306 &     23,284 &    87.16 \\
                       Double If &      4,828 &      1,294 &   309.38 \\
                Duplicate Sprite &    719,309 &     12,357 &    73.67 \\
               Duplicated Script &     14,171 &      6,252 &   148.12 \\
              Empty Control Body &     21,738 &      5,628 &   180.78 \\
              Empty Custom Block &      2,000 &      1,074 &   203.38 \\
                   Empty Project &         27 &         27 &     0.00 \\
                    Empty Script &     24,013 &      9,973 &   116.03 \\
                    Empty Sprite &     25,855 &     11,340 &    53.59 \\
                     Long Script &    136,969 &     33,949 &    75.76 \\
                  Message Naming &    195,099 &     15,781 &    81.41 \\
                      Middle Man &      1,573 &        903 &   342.83 \\
Multiple Attribute Modifications &     10,836 &      3,854 &   169.72 \\
                    Nested Loops &      4,606 &      1,750 &   162.81 \\
  Same Variable Different Sprite &     66,738 &      3,591 &   240.70 \\
              Sequential Actions &      9,249 &      3,086 &   148.33 \\
                   Sprite Naming &    222,603 &     47,708 &    58.15 \\
      Unnecessary If After Until &        974 &        448 &   152.59 \\
                Unnecessary Loop &      4,279 &      1,585 &   165.13 \\
                Unnecessary Time &     25,384 &      3,620 &   173.18 \\
             Unused Custom Block &      8,294 &      2,633 &   193.95 \\
                Unused Parameter &      3,360 &      1,362 &   213.05 \\
                Unused Variables &     70,560 &     12,082 &   121.09 \\
    Variable Initialization Race &      7,134 &      4,724 &   166.52 \\
\bottomrule
\end{tabular}
\end{table}

